Prediction techniques for dynamic imaging with online primal-dual methods

Online optimisation facilitates the solution of dynamic inverse problems, such as image stabilisation, fluid flow monitoring, and dynamic medical imaging. In this paper, we improve upon previous work on predictive online primal-dual methods on two fronts. Firstly, we provide a more concise analysis that symmetrises previously unsymmetric regret bounds, and relaxes previous restrictive conditions on the dual predictor. Secondly, based on the latter, we develop several improved dual predictors. We numerically demonstrate their efficacy in image stabilisation and dynamic positron emission tomography.

==> better_predictmacros.tex <==

\def\filmstripinfocolour{orange!80!black}

\makeatletter

\def\rescalevby#1{%
    \gdef\plotvscaling{#1}%
    \gdef\displacementinfo{%
        \filmstripframecount%
        \node[below right,color=\filmstripinfocolour] at (\filmstrip@framex, \filmstrip@framey) {$#1\times$};%
    }%
}
\def\resetrescalev{%
    \gdef\plotvscaling{1}%
    \global\let\displacementinfo\filmstripframecount%
}
\resetrescalev

\newcommand{\plotvcumul}[2]{
    \fill [black!5] (\filmstrip@framex, \filmstrip@framey) rectangle +(\filmstrip@iw, -\filmstrip@ih);
    \begin{axis}[%
        at={(\filmstrip@framex+\filmstrip@iw/2,\filmstrip@framey-\filmstrip@ih/2)},%
        anchor=origin,%
        width=\filmstrip@iw,%
        height=\filmstrip@ih,%
        hide axis=true,%
        scale mode=none,%
        disabledatascaling=true,%
        scale={\plotvscaling*\filmstrip@iw/2},%
        xmin={-1/\plotvscaling},%
        xmax={1/\plotvscaling},%
        ymin={-0.667/\plotvscaling},%
        ymax={0.667/\plotvscaling},%
        %clip marker paths=true%
    ]
        \addplot[color=orange!50!white,line width=0.5pt,
                 restrict expr to domain={\thisrow{iter}}{1:\frame}]
            table[x=v_cumul_true_x, y=v_cumul_true_y]{#1_hifi.txt};

        \addplot[color=\filmstripinfocolour,line width=0.5pt,
                 restrict expr to domain={\thisrow{iter}}{1:\frame}]
            table[x=v_cumul_true_x, y=v_cumul_true_y]{#1.txt};

        \def\tempa{#2}
        \ifx\tempa\@empty\else
            \addplot[color=blue,line width=0.5pt,
                    restrict expr to domain={\thisrow{iter}}{1:\frame}]
                table[x=v_cumul_est_x, y=v_cumul_est_y]{#1.txt};
        \fi
    \end{axis}
}
\makeatother

%\newcommand{\dostrip}[2][]{%
%    \centering%
%    \ifdraft{%
%        (Removed in draft for compilation speed)%
%    }{%
%        % julia> n=1:6; @. exp(log(30)+(log(1000)-log(30))*(n-1)/5)
%        % 6-element Array{Float64,1}:
%        %   30.000000000000004
%        %   60.49186910982997 
%        %  121.97554094669343 
%        %  245.95094858493624 
%        %  495.934419641283   
%        %  999.9999999999998   
%        \def\nframes{7}%
%        \def\framespec{1/30,2/50,3/100,4/300,5/500,6/1000,7/3000}%
%        \def\striph{0.74\paperheight}%
%        \tikzexternalenable%
%        \subcaptionbox{Noisy}{%
%            \tikzsetnextfilename{#2_data_frames}%
%            \filmstripv{img/#2_data_frame}{\nframes}{\framespec}{\striph}%
%        }%
%        \subcaptionbox{Reconstruction}{%
%            \tikzsetnextfilename{#2_reco_frames}%
%            \filmstripv{img/#2_reco_frame}{\nframes}{\framespec}{\striph}%
%        }%
%        \subcaptionbox{Cumulative displacement}{%
%            \tikzsetnextfilename{#2_displacement}%
%            \filmstripvgen{\plotvcumul{img/#2}{#1}\displacementinfo}%
%                          {\nframes}{\framespec}{\striph}%
%        }%
%        \tikzexternaldisable
%    }
%}



\newcommand{\dostrip}[5][]{%
    \centering%
    \ifdraft{%
        (Removed in draft for compilation speed)%
    }{%
        % julia> n=1:6; @. exp(log(30)+(log(1000)-log(30))*(n-1)/5)
        % 6-element Array{Float64,1}:
        %   30.000000000000004
        %   60.49186910982997 
        %  121.97554094669343 
        %  245.95094858493624 
        %  495.934419641283   
        %  999.9999999999998   
        \def\nframes{7}%
        \def\framespec{1/300,2/1000,3/2000,4/2500,5/3300,6/3500,7/4000}%
        \def\striph{0.74\paperheight}%
        \tikzexternalenable%
        \subcaptionbox{No prediction}{%
            \tikzsetnextfilename{#2_reco_frames}%
            \filmstripvt{img/#2_reco_frame}{\nframes}{\framespec}{\striph}%
        }%
        \subcaptionbox{Proximal (old)}{%
            \tikzsetnextfilename{#3_reco_frames}%
            \filmstripv{img/#3_reco_frame}{\nframes}{\framespec}{\striph}%
        }%
        \subcaptionbox{Zero dual}{%
            \tikzsetnextfilename{#4_reco_frames}%
            \filmstripv{img/#4_reco_frame}{\nframes}{\framespec}{\striph}%
        }%
        \subcaptionbox{Dual scaling}{%
            \tikzsetnextfilename{#5_reco_frames}%
            \filmstripv{img/#5_reco_frame}{\nframes}{\framespec}{\striph}%
        }%
        \tikzexternaldisable
    }
}


%let's try it for denoising
\newcommand{\dostripd}[5][]{%
    \centering%
    \ifdraft{%
        (Removed in draft for compilation speed)%
    }{%
        % julia> n=1:6; @. exp(log(30)+(log(1000)-log(30))*(n-1)/5)
        % 6-element Array{Float64,1}:
        %   30.000000000000004
        %   60.49186910982997 
        %  121.97554094669343 
        %  245.95094858493624 
        %  495.934419641283   
        %  999.9999999999998   
        \def\nframes{9}%
        \def\framespec{1/30,2/100,3/1000,4/2500,5/5000,6/6000,7/8000,8/8700,9/10000}%
        \def\striph{\paperwidth}%
        \tikzexternalenable%
        \subcaptionbox{No prediction}{%
            \tikzsetnextfilename{#2_reco_frames}%
            \filmstripvdt{img/#2_reco_frame}{\nframes}{\framespec}{\striph}%
        }%
        \subcaptionbox{Proximal (old)}{%
            \tikzsetnextfilename{#3_reco_frames}%
            \filmstripvd{img/#3_reco_frame}{\nframes}{\framespec}{\striph}%
        }%
        \subcaptionbox{Zero dual}{%
            \tikzsetnextfilename{#4_reco_frames}%
            \filmstripvd{img/#4_reco_frame}{\nframes}{\framespec}{\striph}%
        }%
        \subcaptionbox{Dual scaling}{%
            \tikzsetnextfilename{#5_reco_frames}%
            \filmstripvd{img/#5_reco_frame}{\nframes}{\framespec}{\striph}%
        }%
        \tikzexternaldisable
    }
}


\newcommand\scinumber[1]{%
    \pgfmathprintnumber[assume math mode=true,sci,sci 10e,precision=2]{#1}%
}

\def\loadEXPPARAMs#1{\input{img/#1_params.tex}}

\pgfplotsset{
    % Plot a graph breaking it at y=#2 into 1/5 tight scaling lower half, and 3/5 loose scaling
    % upper half. #1 and #3 are minimum and maximum of y.
    zoomed/.code n args={3}{
        \pgfmathsetmacro{\YAmin}{#1}
        \pgfmathsetmacro{\YAzoom}{#2}
        \pgfmathsetmacro{\YAmax}{#3}
        \pgfplotsset{
            y coord trafo/.code={%
                % The abs is only needed because pgfmath is junk, and tries to evaluate both arms
                % before even deciding on the condition.
                \pgfmathifthenelse{##1 >= \YAzoom}
                                  {((abs(##1-\YAzoom)/(\YAmax-\YAzoom)))^(1/3)}
                                  {-(abs((##1-\YAzoom)/(\YAmin-\YAzoom)))^(1/3)}

            },
            y coord inv trafo/.code={%
                \pgfmathifthenelse{##1 >= 0}
                                  {(##1^3)*(\YAmax-\YAzoom)+\YAzoom}
                                  {(-##1^3)*(\YAmin-\YAzoom)+\YAzoom}
            },
            extra y ticks = {\YAzoom},
            y axis line style= { draw=none },
            yticklabel style = {xshift=-2ex},
            ylabel style = {yshift=2ex}, % this is reserved, actually shifts x and negatively
            ymax = \YAmax,
            ymin = \YAmin,
            % extra description/.code = {
            %     % Draw zigzag between the two windows
            %     \draw[line width=0.5pt, dashed] (rel axis cs:0,0)
            %         --(rel axis cs:0,0.15)
            %         --(rel axis cs:-0.025,0.175)
            %         --(rel axis cs:0,0.2);
            %     \draw[line width=0.5pt]
            %         (rel axis cs:0,0.2)
            %         --(rel axis cs:0.025,0.225)
            %         --(rel axis cs:0,0.25)
            %         --(rel axis cs:0,1);
            % }
        }
    }
}

